Tree! I am no Tree! I am a Low Dimensional Hyperbolic Embedding

Given data, finding a faithful low-dimensional hyperbolic embedding of the data is a key method by which we can extract hierarchical information or learn representative geometric features of the data. In this paper, we explore a new method for learning hyperbolic representations by taking a metric-first approach. Rather than determining the low-dimensional hyperbolic embedding directly, we learn a tree structure on the data. This tree structure can then be used directly to extract hierarchical information, embedded into a hyperbolic manifold using Sarkar's construction \cite{sarkar}, or used as a tree approximation of the original metric. To this end, we present a novel fast algorithm \textsc{TreeRep} such that, given a $\delta$-hyperbolic metric (for any $\delta \geq 0$), the algorithm learns a tree structure that approximates the original metric. In the case when $\delta = 0$, we show analytically that \textsc{TreeRep} exactly recovers the original tree structure. We show empirically that \textsc{TreeRep} is not only many orders of magnitude faster than previously known algorithms, but also produces metrics with lower average distortion and higher mean average precision than most previous algorithms for learning hyperbolic embeddings, extracting hierarchical information, and approximating metrics via tree metrics.

==> labels.tex <==
\newlabel{sec:understand}{{5}{12}{Metric First Discussion and Justification}{section.5}{}}
\newlabel{sec:proofs}{{6}{12}{Proofs}{section.6}{}}
\newlabel{sec:treerepproofs}{{6.1}{12}{Tree Representation Proofs}{subsection.6.1}{}}
\newlabel{lem:contract}{{4}{13}{}{lem.4}{}}
\newlabel{part:r}{{1}{13}{Tree Representation Proofs}{Item.9}{}}
\newlabel{part:zone1r}{{2}{13}{Tree Representation Proofs}{Item.10}{}}
\newlabel{part:zone1}{{3}{13}{Tree Representation Proofs}{Item.11}{}}
\newlabel{part:zone2}{{4}{14}{Tree Representation Proofs}{Item.12}{}}
\newlabel{defn:zones}{{13}{15}{}{defn.13}{}}
\newlabel{lem:disconnect}{{5}{16}{}{lem.5}{}}
\newlabel{sec:treeaproxproofs}{{6.2}{17}{Tree Approximation Proofs}{subsection.6.2}{}}
\newlabel{sec:acones}{{7}{18}{Geometry: Asymptotic Cones}{section.7}{}}
\newlabel{sec:gtrees}{{8}{19}{Geometry: Geodetic Tree}{section.8}{}}
\newlabel{thm:geodesic1}{{5}{19}{}{thm.5}{}}
\newlabel{def:equiv}{{22}{19}{}{defn.22}{}}
\newlabel{thm:geodesic2}{{6}{19}{}{thm.6}{}}
\newlabel{sec:trbest}{{9}{20}{\textsc {TreeRep} Best}{section.9}{}}
\newlabel{table:best}{{4}{20}{\textsc {TreeRep} Best Numbers}{table.4}{}}
\newlabel{sec:improvedist}{{10}{20}{Improving Distortion}{section.10}{}}
\newlabel{table:heurestic}{{5}{20}{MAP and average distortion for the \textsc {TreeRep} and MST after doing the heuristic optimization. The time taken for both optimizations is the same}{table.5}{}}
\newlabel{sec:expappendix}{{11}{21}{Experiment and Practical Details}{section.11}{}}
\newlabel{def:dist}{{24}{21}{}{defn.24}{}}
\newlabel{def:map}{{25}{21}{}{defn.25}{}}
\newlabel{sec:code}{{12}{23}{Tree Representation Pseudo-code}{section.12}{}}
\newlabel{fig:PTSarich}{{4}{24}{Figure for Sarich data produced by PT code}{figure.4}{}}
\newlabel{fig:sarich}{{5}{24}{Immunological distances from \cite {sarich}}{figure.5}{}}
\newlabel{fig:z12universal}{{6}{24}{Figure showing the placement of the Steiner node $R'$ for the Zone 1 and Zone 2 recursion. The nodes in orange are Steiner nodes and the nodes in green come from the data set $V$}{figure.6}{}}
\newlabel{alg:tree_struct_recurse}{{3}{25}{Tree Representation Pseudo-code}{algorithm.3}{}}
\newlabel{alg:tree_struct2}{{4}{26}{Tree Representation Pseudo-code}{algorithm.4}{}}
\newlabel{table:graph}{{6}{25}{Table with the time taken in seconds, MAP, and average distortion for all of the algorithms when given metrics that come from unweighted graph. Darker cell colors indicates better numbers for MAP and average distortion. The number next to PT, PM, LM is the dimension of the space used to learn the embedding. The numbers for \textsc {TreeRep} (TR) are the average numbers over 20 trials. The table also shows some graph statistics such as $n$, the number of nodes, $m$, the number of edges, and $\delta $, the hyperbolcity of the metric}{table.6}{}}

